Versatile Single-Loop Method for Gradient Estimator: First and Second Order Optimality, and its Application to Federated Learning

While variance reduction methods have shown great success in solving large scale optimization problems, many of them suffer from accumulated errors and, therefore, should periodically require the full gradient computation. In this paper, we present a single-loop algorithm named SLEDGE (Single-Loop mEthoD for Gradient Estimator) for finite-sum nonconvex optimization, which does not require periodic refresh of the gradient estimator but achieves nearly optimal gradient complexity. Unlike existing methods, SLEDGE has the advantage of versatility; (i) second-order optimality, (ii) exponential convergence in the PL region, and (iii) smaller complexity under less heterogeneity of data. We build an efficient federated learning algorithm by exploiting these favorable properties. We show the first and second-order optimality of the output and also provide analysis under PL conditions. When the local budget is sufficiently large and clients are less (Hessian-)~heterogeneous, the algorithm requires fewer communication rounds then existing methods such as FedAvg, SCAFFOLD, and Mime. The superiority of our method is verified in numerical experiments.

==> firstorder.tex <==
% %File: formatting-instruction.tex
% \documentclass[letterpaper]{article}
% \usepackage{aaai}
% \usepackage{bbm}
% \usepackage{times}
% \usepackage{helvet}
% \usepackage{courier}
% \usepackage{mydefs}
% \frenchspacing
% \setlength{\pdfpagewidth}{8.5in}
% \setlength{\pdfpageheight}{11in}
% \pdfinfo{
% /Title Full Gradient at the Initial Point is Necessary and Sufficient for Variance Reduced Nonconvex Optimization
% /Author Kazusato Oko+}
% \setcounter{secnumdepth}{0}

% %%%%%%%%%%%%%%%%%
% \newcommand{\AlgMain}{UltimateSARAH}
% \newcommand{\AlgNumMain}{Algorithm 1\ }
% %%%%%%%%%%%%%%%%%

% \begin{document}
% % The file aaai.sty is the style file for AAAI Press 
% % proceedings, working notes, and technical reports.
% %
% \title{Full Gradient at the Initial Point is Necessary and Sufficient\\ for Variance Reduced Nonconvex Optimization}
% \author{Kazusato Oko+\\
% The University of Tokyo\\
% }
% \maketitle

% \begin{algorithm}[h]\label{alg:main}
%     \caption{\AlgMain$(x_0, \eta, b, T, r)$}
%     \begin{algorithmic}[1]
%         \State{{\bf Option I: }$y^0_i\leftarrow \nabla f_i(x_0) \ (i=1,\cdots,n)$}
%         \State{\hspace{15mm}Randomly sample $b$ data $I_{0}\ (|I_{0}|=b)$}
%         \State{\hspace{15mm}$y^0_i\leftarrow \frac{1}{b}\sum_{i\in I_0}\nabla f_i(x_0)\ (i=1,\cdots,n)$}
%         \State{{\bf Option II: }$y^0_i\leftarrow \nabla f_i(x_0) \ (i=1,\cdots,n)$}
%             \For{$t=1$ to $T$}
%             \State{Randomly sample $b$ data $I_{t}\ (|I_{t}|=b)$}
%             \State{$\displaystyle x_t \leftarrow x_{t-1} - \frac{\eta}{n} \sum_{i=1}^n y^{t-1}_i + \xi_t \quad (\xi_t \sim B(0,r))$}
%             \State{$y^t_{i} \leftarrow \begin{cases}\nabla f_i (x_t) \quad {\rm for\ } j\in I_t \\ \frac1b \sum_{j\in I_t} (\nabla f_j(x_t) - \nabla f_j (x_{t-1}))+ y^{t-1}_{i}\\
%             \hspace{45mm} {\rm for\ } i\notin I_t\end{cases}$}
%             \EndFor
%       \State{\textbf{Output}\ $x_t$ randomly from $t=0,\cdots,T-1$}
%     \end{algorithmic}
% \end{algorithm}

% \begin{assumption}[Gradient Lipschitzness]\label{assumption:gradLipschitz}
% For all $i\in [n]$, $f_i$ is $L$-gradient Lipschitz, i,e, \begin{align}\|\nabla^2 f_i(x) - \nabla f_i(x)\|\leq L\|x-y\|,\quad \forall x,y\in \R^d.\end{align}
% \end{assumption}
% \begin{assumption}[Existence of global infimum]\label{assumption:GlobalInfimum}
% $f$ has a global infimum and $\Delta:=f(x_0)-\inf_{x\in \R^d}f(x)$.
% \end{assumption}
% \begin{assumption}[Boundedness of Gradient at $x_0$]
% \label{assumption:BoundedGradient}
% We let $G:=\frac1n \sum_{i=1}^n \|\nabla f_i(x_0)\|^2$.
% \end{assumption}
% \begin{assumption}[Hessian Heterogeneity]\label{assumption:heterogeneity}
% $\{f_i\}_{i=1}^n$ is second-order $\zeta$-heterogeneous, i,e, for any $i,j\in [n]$ and $x\in \R^d$, \begin{align}\|\nabla^2 f_i(x) - \nabla^2 f_j(x)\|\leq \zeta.\end{align}
% \end{assumption}

% \onecolumn
% \section{Finding First-order Stationary Points with High Probability}

% \begin{theorem}\label{theorem:First-Main}
% Under \cref{assumption:gradLipschitz,assumption:GlobalInfimum,assumption:BoundedGradient}, if we choose
% $b = \Theta\left(\sqrt{n}\right), \eta = \tilde{\Theta} \left(\frac{1}{L}\right) \text{ and } r = O\left(\frac{\eps}{L}\right)$,
% \AlgNumMain with Option I finds an $\eps$-first-order stationary point for problem \cref{eq:TargetFiniteSum} using
% \begin{align}
%     \tilde{O}\left(\frac{(L\Delta + G) \sqrt{n}}{\eps^2} \right)
% \end{align}
% stochastic gradients with probability at least $1-O(\delta)$.

% Moreover, under \cref{assumption:gradLipschitz,assumption:GlobalInfimum,assumption:heterogeneity}, if we choose
% $b = \Theta\left(\frac{\zeta}{L}\sqrt{n}\right)\geq 1, \eta = \Theta \left(\frac{1}{L}\right) \text{ and } r = O\left(\frac{\eps}{L}\right)$,
% \AlgNumMain with Option II finds an $\eps$-first-order stationary point for problem \cref{eq:TargetFiniteSum} using
% \begin{align}
%     \tilde{O}\left(n + \frac{\zeta \Delta \sqrt{n}}{\eps^2} \right)
% \end{align}
% stochastic gradients with probability at least $1-O(\delta)$.
% \end{theorem}

% First, we make use of the classical argument found in \ref{}, that ensures decrease of the function values.
% Let $f$ be an $L$-Gradient Lipschitz function and $x_t:=x_{t-1}-\eta v_{t-1}+\xi_{t-1}$ with $\|\xi_{t-1}\|\leq r$.
% \begin{align}
%     f(x_t)
%     & \leq 
%     f(x_{t-1}) + \langle \nabla f(x_{t-1}), x_t-x_{t-1}\rangle + \frac{L}{2}\|x_t-x_{t-1}\|^2
%     \\ & =    
%     f(x_{t-1}) + \left\langle \nabla f(x_{t-1}) - v_{t-1} + \frac{\xi_{t-1}}{\eta}, x_t-x_{t-1}\right\rangle +
%     \left\langle  v_{t-1} - \frac{\xi_{t-1}}{\eta}, x_t-x_{t-1}\right\rangle
%     + \frac{L}{2}\|x_t-x_{t-1}\|^2
%     \\ &  =      
%     f(x_{t-1}) + \left\langle \nabla f(x_{t-1}) - v_{t-1} + \frac{\xi_{t-1}}{\eta}, x_t-x_{t-1}\right\rangle 
%     - \left(\frac{1}{\eta}-\frac{L}{2}\right)\|x_t-x_{t-1}\|^2
%     \\ &\label{eq:First-FunctionDecrease-1} = 
%     f(x_{t-1}) + \frac{\eta}{2} \left\| \nabla f(x_{t-1}) - v_{t-1} + \frac{\xi_{t-1}}{\eta}\right\|^2
%     - \frac{\eta}{2}\|\nabla f(x_{t-1})\|^2
%     - \left(\frac{1}{2\eta}-\frac{L}{2}\right)\|x_t-x_{t-1}\|^2
%     \\ & \label{eq:First-FunctionDecrease-2} \leq
%     f(x_{t-1}) + \eta \|\nabla f(x_{t-1}) - v_{t-1}\|^2
%     - \frac{\eta}{2}\|\nabla f(x_{t-1})\|^2
%     - \left(\frac{1}{2\eta}-\frac{L}{2}\right)\|x_t-x_{t-1}\|^2
%     + \eta \left\|\frac{\xi_{t-1}}{\eta}\right\|^2
%      \\ & \label{eq:First-FunctionDecrease-3} \leq
%     f(x_{t-1}) + \eta \|\nabla f(x_{t-1}) - v_{t-1}\|^2
%     - \frac{\eta}{2}\|\nabla f(x_{t-1})\|^2
%     - \left(\frac{1}{2\eta}-\frac{L}{2}\right)\|x_t-x_{t-1}\|^2
%     + \frac{r^2}{\eta},
% \end{align}
% where we used $x_t-x_{t-1}=\eta v_{t-1}+\xi_{t-1}$ and $\langle a-b,b\rangle=\frac12 (\|a-b\|^2-\|a\|^2+\|b\|^2)$ for \eqref{eq:First-FunctionDecrease-1}, $\|a+b\|^2\leq 2(\|a\|^2+\|b\|^2)$ for \eqref{eq:First-FunctionDecrease-2}, and $\|\xi_{t-1}\|\leq r$ for \eqref{eq:First-FunctionDecrease-3}.
% \\

% Our algorithm uses $v_t = \frac1n\sum_{i=1}^n y^t_i$ as an estimator of $\nabla f(x_t)$.
% From now, we show that the variance term $\|v_t - \nabla f(x_{t})\|^2$ is bounded with high probability.

% \begin{lemma}\label{lemma:First-VarianceBound}
% Let $v_t = \frac1n\sum_{i=1}^n y^t_i$ and all the other variables be as stated in \cref{alg:main}.
% Then, there exist $t_0 = \tilde{\Theta}\left(\frac{n}{b}\right)$ and an absolute constant $C_1 = \tilde{O}(1)$ such that
% \begin{align}
%     \|v_t - \nabla f(x_t)\|^2
%     \leq
%     \frac{C_1}{\sqrt{n}}
%     \left(\zeta^2\sum_{s =\max\{1,t-t_0+1\}}^{t}\|x_s -x_{s -1}\|^2 + \mathbbm{1}[t< t_0]\cdot G\right)
% \end{align}
% holds for all $t=0,\cdots,T$ with probability at least $1-O(\delta)$.
% \end{lemma}
% \begin{proof}
% For each $s,t\geq 1$, we let $J_s^t = [n]\setminus \bigcup_{\tau = s}^t I_t$, which is a set of indexes that are not selected between $s$ and $t$.
% Then, $\|v_t - \nabla f(x_{t})\|^2$ is written as
% \begin{align}
% \label{eq:First-Variance-1}
%     v_t - \nabla f(x_{t}) = \frac{1}{n} \sum_{s=1}^t \left( \frac{|J_s^t|}{b}\sum_{i\in I_s} (\nabla f_i(x_{s})-\nabla f_i(x_{s-1}))
%     - \sum_{i\in J_s^t}(\nabla f_i(x_{s})-\nabla f_i(x_{s-1}))
%     \right)+\frac{1}{n}\sum_{i\in J_1^t}(y^0_i-\nabla f_i(x_0))
% .
% \end{align}
% The simple but important observation is that if $t-s$ is as sufficiently large as $\tilde{O}(\sqrt{n})$, every $f_i$ is sampled at least once between $s$ and $t$ with high probability.
% Owing to this fact, we can cut off the errors caused $\tilde{O}(\sqrt{n})$ steps before.
% Indeed, for each $f_i$ and $\delta>0$, the probability that $f_i$ is not sampled between $s$ and $t$ is bounded as
% \begin{align}
%     \label{eq:First-Variance-2}
%     \left(1-\frac{b}{n}\right)^{t-s+1}
%     \leq
%     \left(1-\frac{b}{n}\right)^{\frac{n}{b}\cdot \frac{b(t-s+1)}{n}}
%     \leq
%     \exp \left(- \frac{b(t-s+1)}{n}\right)
%     .
% \end{align}
% By taking $t-s+1=\Omega\left(\frac{n}{b}\log \frac{nT}{\delta}\right)$, the right-hand side of \eqref{eq:First-Variance-2} is bounded by $\frac{\delta}{nT}$.
% This means that, when $t\geq t_0$,$\bigcup_{t=t-t_0+1}^t I_t$ covers $[n]$ with probability $1-\frac{\delta}{T}$.
% %, or equivalently, $J_{t-t_0}^t = \emptyset$ holds. 
% Thus, with probability at least $1-\delta$, $J_{s}^t = \emptyset$ holds for every $t$ and $s\leq t-t_0$ and below we consider the events where this happens.
% %The main difficulty is that $J_s^t$ is not independent for each $s=t_0,\cdots,t$.
% %To overcome this, we iteratively separate the term $\sum_{i\in J_s^t}(\nabla f_i(x_{s})-\nabla f_i(x_{s-1}))$ from the others, as follows.

% Then, $\|v_t - \nabla f(x_{t})\|^2$ is decomposed as follows.
% \begin{align}
%     & \|v_t - \nabla f(x_{t})\|^2
%     \\ & =
%     \left\|
%         \frac{1}{n} \sum_{s=\max\{1,t-t_0+1\}}^t \left( \frac{|J_s^t|}{b}\sum_{i\in I_s} (\nabla f_i(x_{s})-\nabla f_i(x_{s-1}))
%     -
%     \sum_{i\in J_s^t}(\nabla f_i(x_{s})-\nabla f_i(x_{s-1}))
%     \right)+\frac{\mathbbm{1}[t\leq t_0]}{n}\sum_{i\in J_1^t}(y^0_i-\nabla f_i(x_0))
%     \right\|^2
%     \\ & = 
%     \left\|
%     \frac{1}{n} \sum_{s=\max\{1,t-t_0+1\}}^t \left( \frac{|J_s^t|}{b}\sum_{i\in I_s} (\nabla f_i(x_{s})-\nabla f_i(x_{s-1}))
%     -
%     \sum_{i\in J_s^t}(\nabla f_i(x_{s})-\nabla f_i(x_{s-1}))
%     \right)+\frac{\mathbbm{1}[t\leq t_0]}{n}\sum_{i\in J_1^t}(y^0_i-\nabla f_i(x_0))
%     \right\|^2
%     \\ & \leq
%     3\underbrace{
%     \left\|
%     \frac{1}{n} \sum_{s=\max\{1,t-t_0+1\}}^t \sum_{i\in J_s^t}(\nabla f_i(x_{s})-\nabla f_i(x_{s-1}) - (\nabla f(x_{s})+\nabla f(x_{s-1})))\right\|^2 
%     }_{\rm (a)}
%     \\ & \hspace{3.5mm}
%     + 
%     3\underbrace{
%     \left\|\frac{1}{n}\sum_{s=\max\{1,t-t_0+1\}}^t\frac{|J_s^t|}{b}\sum_{i\in I_s} (\nabla f_i(x_{s})-\nabla f_i(x_{s-1})- (\nabla f(x_{s})+\nabla f(x_{s-1})))\right\|^2
%     }_{\rm (b)}
%     +3\underbrace{
%     \left\|\frac{\mathbbm{1}[t\leq t_0]}{n}\sum_{i\in J_1^t}(y^0_i-\nabla f_i(x_0))
%     \right\|^2
%      }_{\rm (c)}
% \end{align}

% We bound each term with high probability, using the concentration inequalities.
% \\

% \noindent {\bf Bounding (a)}\\
% First, we consider (a).
% We regard $t$ and $J_s^t$ as fixed.
% It is not difficult to see
% \begin{align}
%     &
%     \left\|
%     \frac{1}{n} \sum_{s=\max\{1,t-t_0+1\}}^t \sum_{i\in J_s^t}(\nabla f_i(x_{s})-\nabla f_i(x_{s-1}) - (\nabla f(x_{s})+\nabla f(x_{s-1})))\right\|^2 
%     \\ & \leq
%     \frac{t_0}{n^2}\sum_{s=\max\{1,t-t_0+1\}}^t
%     \left\|
%      \sum_{i\in J_s^t}(\nabla f_i(x_{s})-\nabla f_i(x_{s-1}) - (\nabla f(x_{s})+\nabla f(x_{s-1})))\right\|^2 
% \end{align}
% holds. 
% For each $s$, from assumption \cref{assumption:heterogeneity} (or setting $\zeta = 2L$), we get
% \begin{align}
%     R = \|\nabla f_i(x_{s})-\nabla f_i(x_{s-1}) - (\nabla f(x_{s})+\nabla f(x_{s-1}))\|
%     \leq
%     \zeta \|x_s-x_{s-1}\|
% \end{align}
% for all $i\in J_s^t$.
% % Moreover, using the formula for sampling without replacement,
% % \begin{align}
% %     \sigma^2 & = \mathbb{E}_{|J_s^t|:{\rm fix}}\left[\left\|
% %      \sum_{i\in J_s^t}(\nabla f_i(x_{s})-\nabla f_i(x_{s-1}) - (\nabla f(x_{s})+\nabla f(x_{s-1})))\right\|^2 \right]
% %     \\ & \leq
% %     \frac{(n-|J_s^t|)|J_s^t|}{(n-1)}\zeta^2 \|x_s-x_{s-1}\|^2
% %     \leq
% %     \zeta^2|J_s^t|\|x_s-x_{s-1}\|^2  
% % \end{align}
% % holds, here $\mathbb{E}_{|J_s^t|:{\rm fix}}$ means conditional expectation on the choice of $J_s^t$, with its size $J_s^t$ fixed.

% Then, we apply Hoeffding's inequality without replacement (\cref{proposition:Bernstein-vector}) to get
% \begin{align}
%     \mathbb{P}\left[
%      \left\|
%      \sum_{i\in J_s^t}(\nabla f_i(x_{s})-\nabla f_i(x_{s-1}) - (\nabla f(x_{s})+\nabla f(x_{s-1})))\right\|^2
%      \geq 
%     \right]
% \end{align}
% \end{proof}

% \begin{proof}[Proof of \cref{theorem:First-Main}]
% Finally, we show the first-order convergence of \AlgNumMain.
% We evaluate $f(x_t)+ \frac{n}{bL}\|v_t - \nabla f(x_t)\|^2$ in full expectation.
% Applying \cref{eq:First-FunctionDecrease-3} and \cref{lemma:First-VarianceBound}, we have that
% \begin{align}
%     &
%     \mathbb{E}\left[f(x_t)+ \frac{n}{bL}\|v_t - \nabla f(x_t)\|^2\right]
%     \\ & \leq
%     \mathbb{E}\left[
%     f(x_{t-1}) + \left(\eta + \frac{n}{bL} - \frac{1}{L}\right)\| v_{t-1} - \nabla f(x_{t-1})\|^2
%     - \frac{\eta}{2}\|\nabla f(x_{t-1})\|^2
%     - \left(\frac{1}{2\eta}-\frac{L}{2}-\frac{n\zeta^2}{b^2 L}
% \right)\|x_t-x_{t-1}\|^2
%     + \frac{r^2}{\eta}
%     \right]
% \end{align}
% for $t=1,2,\cdots,T$.

% With Option I, we choose $b\geq \sqrt{n}$ and $\eta \leq \frac{1}{9L}$, so that $\eta + \frac{n}{bL} - \frac{1}{L}\leq \frac{n}{bL}$ and $\frac{1}{2\eta}-\frac{L}{2}-\frac{n\zeta^2}{b^2 L}\geq \frac{9L}{2}-\frac{L}{2} - 4L=0$ holds. 
% With Option II, we choose $b\geq \frac{\zeta}{L}\sqrt{n}$ and $\eta \leq \frac{1}{3L}$, so that $\eta + \frac{n}{bL} - \frac{1}{L}\leq \frac{n}{bL}$ and $\frac{1}{2\eta}-\frac{L}{2}-\frac{n\zeta^2}{b^2 L}\geq \frac{3L}{2}-\frac{L}{2} - L=0$ holds.
% Thus, in both cases, for all $t=1,2,\cdots,T$, we obtain
% \begin{align}
%     \mathbb{E}\left[f(x_t)+ \frac{n}{bL}\|v_t - \nabla f(x_t)\|^2\right]
%     \leq
%     \mathbb{E}\left[
%     f(x_{t-1}) + \frac{n}{bL}\| v_{t-1} - \nabla f(x_{t-1})\|^2
%     - \frac{\eta}{2}\|\nabla f(x_{t-1})\|^2
%     + \frac{r^2}{\eta}
%     \right].
% \end{align}
% Summing up over $t=1,2,\cdots,T$ and rearranging terms yields
% \begin{align}
%     \mathbb{E}\left[\sum_{t=0}^{T-1}\|\nabla f(x_{t})\|^2\right]
%     & \leq
%     \frac{1}{\eta}
%     \mathbb{E}\left[
%     f(x_0) - f(x_T) + \frac{n}{bL}\| v_{0} - \nabla f(x_{0})\|^2
%     - \frac{n}{bL}\|v_T - \nabla f(x_T)\|^2
%     \right]
%     + \frac{Tr^2}{\eta^2}
%     \\ & \leq 
%     \frac{\Delta}{\eta} + 
%     \frac{1}{\eta}\mathbb{E}\left[
%     \frac{n}{bL}\| v_{0} - \nabla f(x_{0})\|^2
%     \right]
%     + \frac{Tr^2}{\eta^2}
%     .
% \end{align}
% We take $r\leq \frac{\eta \eps}{\sqrt{2}}$, when $\frac{Tr^2}{\eta^2}$ is bounded by $\frac{T\eps^2}{2}$.
% Thus, choosing $x_t$ as an output uniformly from $t=0,1,\cdots,T-1$ with $T\geq \frac{1}{2\eps^2}\left(\frac{\Delta}{\eta} + 
%     \frac{1}{\eta}\mathbb{E}\left[
%     \frac{n}{bL}\| v_{0} - \nabla f(x_{0})\|^2
%     \right]\right)$, the output $\tilde{x}$ satisfies
% $
%     \mathbb{E}\left[\|\nabla f(\tilde{x})\|^2\right]
%     \leq
%     \frac{\eps^2}{2} + \frac{\eps^2}{2} = \eps^2
% $.
    
% When we take Option I, 
% \begin{align}
%     \mathbb{E}\left[\|v_{0} - \nabla f(x_{0})\|^2\right]
%     \leq 
%      \mathbb{E}\left[\left\|\frac{1}{b}\sum_{i\in I_0} \nabla f_i(x_{0}) - \frac{1}{n}\sum_{i=1}^n \nabla f_i(x_{0})\right\|^2\right]
%      \leq
%      \frac{1}{b}\frac{1}{n}\sum_{i=1}^n \|\nabla f_i(x_{0})\|^2 = G
%     .
% \end{align}
% holds by using the fact that $\mathbb{E}[\|X-\mathbb{E}[X]\|^2]\leq \mathbb{E}[\|X\|^2]$ for any random variable $X$.
% Here, the total number of gradient computation can be bounded by
% \begin{align}
% T \cdot \sqrt{n} = O\left(
% \frac{1}{\eps^2}\left(\frac{\Delta}{\eta} + 
%     \frac{1}{\eta}\mathbb{E}\left[
%     \frac{n}{bL}\| v_{0} - \nabla f(x_{0})\|^2
%     \right]\right) \cdot \sqrt{n}\right)
%     =
% O\left(\frac{(L\Delta + G) \sqrt{n}}{\eps^2} \right)
% .
% \end{align}

% On the other hand, when we take Option II, $\|v_{0} - \nabla f(x_{0})\|^2$=0 holds. Thus, the total number of gradient computation can be bounded by
% \begin{align}
% T \cdot \frac{\zeta}{L}\sqrt{n} + n =
% O\left(\frac{\zeta\Delta\sqrt{n}}{\eps^2} + n\right)
% .
% \end{align}
% \end{proof}

% \section{Finding Second-order Stationary Points}

% \subsection{High probability Bound}

% \end{document}
